Hydras for $\omega_{1}$

In this paper we introduce a hydra battle. Each hydra will eventually die out, but the fact is not provable in a set theory with urelements of natural numbers and the assumption that `there exists an uncountable regular ordinal'.

==> header.tex <==


\newcommand{\blem}{\begin{lemma}}
\newcommand{\elem}{\end{lemma}}
\newcommand{\bth}{\begin{theorem}}
\newcommand{\ethm}{\end{theorem}}
\newcommand{\benu}{\begin{enumerate}}
\newcommand{\eenu}{\end{enumerate}}
\newcommand{\bdes}{\begin{description}}
\newcommand{\edes}{\end{description}}
\newcommand{\bdf}{\begin{definition}}
\newcommand{\edf}{\end{definition}}
\newcommand{\bcor}{\begin{cor}}
\newcommand{\ecor}{\end{cor}}
\newcommand{\bprp}{\begin{proposition}}
\newcommand{\eprp}{\end{proposition}}
\newcommand{\bmlem}{\begin{mlemma}}
\newcommand{\emlem}{\end{mlemma}}
\newcommand{\bclm}{\begin{claim}}
\newcommand{\eclm}{\end{claim}}
\newcommand{\bprf}{{\bf Proof}.\hspace{2mm}}
\newcommand{\bitprf}{{\it Proof}.\hspace{2mm}}
\newcommand{\eprf}{\hspace*{\fill} $\Box$}
\newcommand{\eremark}{\hspace*{\fill} {\it End of Remark}}
\newcommand{\edigression}{\hspace*{\fill} {\it End of Digression}}
\newcommand{\eprfclm}{\hspace*{\fill} {\it End of Proof of Claim}}
\newcommand{\eprfcor}{\hspace*{\fill} {\it End of Proof of Corollary}}
\newcommand{\eprfprp}{\hspace*{\fill} {\it End of Proof of Proposition}}
\newcommand{\ovl}{\overline}
\newcommand{\beqn}{\begin{equation}}
\newcommand{\eeqn}{\end{equation}}
\newcommand{\beqnarr}{\begin{eqnarray}}
\newcommand{\eeqnarr}{\end{eqnarray}}
\newcommand{\beqnarrs}{\begin{eqnarray*}}
\newcommand{\eeqnarrs}{\end{eqnarray*}}
\newcommand{\ull}{\underline{\ll}}
\newcommand{\smlskp}{\\ \smallskip \\}
\newcommand{\spand}{\,\&\,}
\newcommand{\udl}{\underline}
\newcommand{\prpr}{\prec\!\!\prec}
\newcommand{\prpreq}{\underline{\prec\!\!\prec}}
\newcommand{\sbsb}{\subset\!\!\subset}
\newcommand{\dcup}{\dot{\cup}}
\newcommand{\dbcup}{\dot{\bigcup}}
\newcommand{\bfm}{\boldmath}
\newcommand{\bfr}{\mbox{\boldmath$r$} }
\newcommand{\bfG}{\mbox{\boldmath$G$} }
\newcommand{\bfZ}{\mbox{\boldmath$Z$} }
\newcommand{\pincl}{\stackrel{\displaystyle \subset}{\scriptstyle \neq}}
\newcommand{\dbigvee}{\bigvee\mbox{\hspace{-2mm}}\bigvee}
\newcommand{\dbigwedge}{\bigwedge\mbox{\hspace{-2mm}}\bigwedge}
\newcommand{\barq}{\bar{q}}
\newcommand{\barr}{\bar{r}}

\newcommand{\Real}{\mathbb{R}}
%\newcommand{\Natural}{\mathbb{N}}
\newcommand{\Rational}{\mathbb{Q}}
\newcommand{\Integer}{\mathbb{Z}}
\newcommand{\Complex}{\mathbb{C}}


\newcommand{\restrict}{\!\upharpoonright\!}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{mlemma}[theorem]{Main Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{cyantheorem}{Theorem}


\newcommand{\alp}{\alpha}
\newcommand{\eps}{\epsilon}
\newcommand{\veps}{\varepsilon}
\newcommand{\del}{\delta}
\newcommand{\Del}{\Delta}
\newcommand{\ome}{\omega}
\newcommand{\Ome}{\Omega}
\newcommand{\bet}{\beta}
\newcommand{\gam}{\gamma}
\newcommand{\Gam}{\Gamma}
\newcommand{\kap}{\kappa}
\newcommand{\sig}{\sigma}
\newcommand{\Sig}{\Sigma}
\newcommand{\tht}{\theta}
\newcommand{\Tht}{\Theta}
\newcommand{\lam}{\lambda}
\newcommand{\Lam}{\Lambda}
\newcommand{\vphi}{\varphi}
\newcommand{\bvphi}{\bar{\varphi}}
\newcommand{\dotveps}{\dot{\veps}}
\newcommand{\fal}{\forall}
\newcommand{\exi}{\exists}
\newcommand{\rarw }{\rightarrow}
\newcommand{\Rarw }{\Rightarrow}
\newcommand{\larw}{\leftarrow}
\newcommand{\Larw}{\Leftarrow}
\newcommand{\lrarw}{\leftrightarrow}
\newcommand{\Lrarw}{\Leftrightarrow}
\newcommand{\uarw}{\uparrow}
\newcommand{\darw}{\downarrow}
\newcommand{\rarwa}{\rightarrow^{A}}
\newcommand{\rarweqa}{\rightarrow^{A}_{=}}
\newcommand{\hkrarw}{\hookrightarrow}
\newcommand{\cala}{{\cal A}}
\newcommand{\calb}{{\cal B}}
\newcommand{\calc}{{\cal C}}
\newcommand{\cald}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calf}{{\cal F}}
\newcommand{\calg}{{\cal G}}
\newcommand{\calh}{{\cal H}}
\newcommand{\cali}{{\cal I}}
\newcommand{\calr}{{\cal TR}}
\newcommand{\caltr}{{\cal R}}
\newcommand{\cals}{{\cal S}}
\newcommand{\calt}{{\cal T}}
\newcommand{\calu}{{\cal U}}
\newcommand{\calv}{{\cal V}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calk}{{\cal K}}
\newcommand{\calm}{{\cal M}}
\newcommand{\caln}{{\cal N}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calo}{{\cal O}}
%\newcommand{\calr}{{\cal R}}
\newcommand{\calw}{{\cal W}}
\newcommand{\calx}{{\cal X}}
\newcommand{\caly}{{\cal Y}}
\newcommand{\calz}{{\cal Z}}
\newcommand{\bfN}{\mbox{\boldmath$N$}}
\newcommand{\bfO}{\mbox{\boldmath$O$}}
\newcommand{\st}{\star}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\lc}{\lceil}
\newcommand{\rc}{\rceil}
\newcommand{\rk}{\mbox{{\rm rk}}}

\newcommand{\sfv}{{\sf v}}
\newcommand{\sfe}{{\sf e}}
\newcommand{\sfsc}{{\sf SC}}
\newcommand{\sfk}{{\sf k}}

\newcommand{\msten}{\mbox{\hspace{10mm}}}
\newcommand{\msfiv}{\mbox{\hspace{5mm}}}
\newcommand{\bfB}{\mbox{\boldmath$B$} }
\newcommand{\setm}{\setminus}
\newcommand{\incl}{\subseteq}
\newcommand{\sqs }{\sqsubset}
\newcommand{\sqse }{\sqsubseteq}
\newcommand{\chkt}{\check{t}}
\newcommand{\chks}{\check{s}}
\newcommand{\tilt}{\tilde{t}}
\newcommand{\precp}{\prec^{+}}
\newcommand{\preceqp}{\preceq^{+}}
\newcommand{\preca}{\prec^{A}}
\newcommand{\preceqa}{\preceq^{A}}
\newcommand{\precb}{\prec^{B}}
\newcommand{\preceqb}{\preceq^{B}}
\newcommand{\precpa}{\prec^{+A}}
\newcommand{\preceqpa}{\preceq^{+A}}
\newcommand{\mmid}{\!\mid\!}
\newcommand{\mdfsubtr}{\mbox{$-$\raisebox{0.8ex}{$\hskip-1.2ex\cdot$}}\,}

